Neighbor-Aware Calibration of Segmentation Networks with Penalty-Based Constraints

Ensuring reliable confidence scores from deep neural networks is of paramount significance in critical decision-making systems, particularly in real-world domains such as healthcare. Recent literature on calibrating deep segmentation networks has resulted in substantial progress. Nevertheless, these approaches are strongly inspired by the advancements in classification tasks, and thus their uncertainty is usually modeled by leveraging the information of individual pixels, disregarding the local structure of the object of interest. Indeed, only the recent Spatially Varying Label Smoothing (SVLS) approach considers pixel spatial relationships across classes, by softening the pixel label assignments with a discrete spatial Gaussian kernel. In this work, we first present a constrained optimization perspective of SVLS and demonstrate that it enforces an implicit constraint on soft class proportions of surrounding pixels. Furthermore, our analysis shows that SVLS lacks a mechanism to balance the contribution of the constraint with the primary objective, potentially hindering the optimization process. Based on these observations, we propose NACL (Neighbor Aware CaLibration), a principled and simple solution based on equality constraints on the logit values, which enables to control explicitly both the enforced constraint and the weight of the penalty, offering more flexibility. Comprehensive experiments on a wide variety of well-known segmentation benchmarks demonstrate the superior calibration performance of the proposed approach, without affecting its discriminative power. Furthermore, ablation studies empirically show the model agnostic nature of our approach, which can be used to train a wide span of deep segmentation networks.

==> Makefile <==
CC = latexmk
CFLAGS = -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make

.PHONY: all clean deep_clean

PDFS = main.pdf
TEX = $(PDFS:.pdf=.tex)
BBL = $(PDFS:.pdf=.bbl)

FIGS = figures/labels.jpg figures/margins.jpg \
	figures/deepcut_proposals.jpg figures/cherry.jpg
LOGFIGS = figures/extended_log_barrier.png figures/log_barrier.png \
	figures/quadra_relu.png figures/derivative.png

all: $(PDFS)

figs: $(FIGS)

main.bbl: main.pdf
%.pdf: %.tex $(FIGS) $(LOGFIGS)
	$(CC) $(CFLAGS) $<
# 	pdflatex $<
# 	pdflatex $<
# 	pdflatex $<

$(FIGS): figues.py
	python $<

$(LOGFIGS) &: log_plots.py
	python $<

# figures/margins.jpg: figues.py
# 	python $<

toto:
	rm -f results/prostate/val_3d_dsc.png && make -f prostate.make results/prostate/val_3d_dsc.png TRN="results/prostate/fs results/prostate/box_prior_box_size_neg_size_noaug results/prostate/box_prior_box_size_neg_ce results/prostate/deepcut" DEBUG='--fontsize 16 --ylabel DSC --figsize 9 6 --labels "Full supervision" "Ours (masked emptiness constraint" "Ours (masked cross-entropy)" "DeepCut" --loc "lower right" --title "PROMISE12 validation dice over time" --colors c r g b'

	rm -f results/prostate/tra_dice.png && make -f prostate.make results/prostate/tra_dice.png TRN="results/prostate/fs results/prostate/box_prior_box_size_neg_size_noaug results/prostate/box_prior_box_size_neg_ce results/prostate/deepcut" DEBUG='--fontsize 16 --ylabel 3D-DSC --figsize 9 6 --labels "Full supervision" "Ours (masked emptiness constraint" "Ours (masked cross-entropy)" "DeepCut" --loc "lower right" --title "PROMISE12 training dice over time" --colors c r g b'

	rm -f results/atlas/val_3d_dsc.png && make -f atlas.make results/atlas/val_3d_dsc.png TRN="results/atlas/ce results/atlas/box_prior_box_size_neg_size results/atlas/box_prior_negative_ce_box_size results/atlas/deepcut" DEBUG='--fontsize 16 --ylabel DSC --figsize 9 6 --labels "Full supervision" "Ours (masked emptiness constraint" "Ours (masked cross-entropy)" "DeepCut" --loc "lower right" --title "ATLAS validation dice over time" --colors c r g b'

# 	rm -f results/prostate/tra_dice.png && make -f prostate.make results/prostate/tra_dice.png TRN="results/prostate/fs results/prostate/box_prior_box_size_neg_size results/prostate/box_prior_box_size_neg_ce" DEBUG="--fontsize 16"
# 	rm -f results/atlas/val_dice.png && make -f atlas.make results/atlas/val_dice.png TRN="results/atlas/ce results/atlas/box_prior_box_size_neg_size results/atlas/deepcut" DEBUG='--fontsize 16 --ylabel 3D-DSC --figsize 10 8 --labels "Full supervision" "Ours (masked emptiness constraint" "DeepCut" --loc "lower right" --title "ATLAS validation 2D-DSC over time" --colors c r b'

clean:
	$(CC) -c
	rm -f *.nav *.snm

deep_clean: clean
	rm -f arxiv.zip $(PDFS) $(BBL)


